The properties and kinematics of HCN emission across the closest starburst galaxy NGC 253 observed with ALMA

Studying molecular gas in nearby galaxies using hydrogen cyanide (HCN) as a tracer for higher densities than CO emission still poses a significant challenge. Even though several galaxies have HCN maps on a few kpc scales, higher-resolution maps are still required. Our goal is to examine the contrast in intensity between two tracers that probe different density regimes - HCN(1-0)/CO(2-1) ratio - and their kinematics across NGC 253. By utilizing the advanced capabilities of the Atacama Large Millimeter/submillimeter Array (ALMA), we can map these features at high resolution across a large field of view and uncover the nature of such dense gas in extragalactic systems. We present new ALMA Atacama Compact Array and Total Power (ACA+TP) observations of the HCN emission across NGC 253, covering the inner 8.6' of the galaxy disk at 300 pc scales. We analyze the integrated intensity and mean velocity of HCN and CO along each line of sight and use SCOUSE software to perform spectral decomposition, which considers each velocity component separately. Molecular gas traced by HCN piles up in a ring-like structure at a radius of 2 kpc. The HCN emission is enhanced by 2 orders of magnitude in the central 2 kpc regions, beyond which its intensity decreases with increasing galactocentric distance. The number of components in the HCN spectra shows a robust environmental dependence, with multiple velocity features across the center and bar. We have identified an increase in the HCN/CO ratio in these regions, corresponding to a velocity component likely associated with a molecular outflow. We have also discovered that the ratio between the total infrared luminosity and dense gas mass, which indicates the star formation efficiency of dense gas, is anti-correlated with the molecular gas surface density up to approximately 200 Msul/pc^2. In contrast, beyond this point, the ratio starts to increase.

==> Tables/obs_lines.tex <==
\begin{table}
\centering
\caption{The summary of ALMA ACA observations of HCN\Jone\, emission at the rest frequency of 88.63\,GHz: the beam size, channel width, and the rms. }
\begingroup
\setlength{\tabcolsep}{8pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.2} % Default value: 1
\begin{tabular}{lcccccc}
\hline \hline \\
Line & Transition & $B_\mathrm{maj}$ & $B_\mathrm{min}$ & $BPA$ {[}deg{]} & $\Delta\upsilon$ & $rms$  \\
 &   & {[}''{]}   &  {[}''{]}   & {[}deg{]} & {[}km s$^{-1}${]} & {[}mK{]}   \\ 
\hline \\
%HCN           & 1 - 0      & 3.68         & 630.20     & 12.40  & &  &                          \\
HCN & \Jone & 21.40 & 10.36 & 83.51 & 1.65 & 6.98 \\
\hline \hline 
\end{tabular}
\endgroup
\label{tab:HCN_obs}
\end{table}
